Deconstructing Generative Adversarial Networks

We deconstruct the performance of GANs into three components: 1. Formulation: we propose a perturbation view of the population target of GANs. Building on this interpretation, we show that GANs can be viewed as a generalization of the robust statistics framework, and propose a novel GAN architecture, termed as Cascade GANs, to provably recover meaningful low-dimensional generator approximations when the real distribution is high-dimensional and corrupted by outliers. 2. Generalization: given a population target of GANs, we design a systematic principle, projection under admissible distance, to design GANs to meet the population requirement using finite samples. We implement our principle in three cases to achieve polynomial and sometimes near-optimal sample complexities: (1) learning an arbitrary generator under an arbitrary pseudonorm; (2) learning a Gaussian location family under TV distance, where we utilize our principle provide a new proof for the optimality of Tukey median viewed as GANs; (3) learning a low-dimensional Gaussian approximation of a high-dimensional arbitrary distribution under Wasserstein distance. We demonstrate a fundamental trade-off in the approximation error and statistical error in GANs, and show how to apply our principle with empirical samples to predict how many samples are sufficient for GANs in order not to suffer from the discriminator winning problem. 3. Optimization: we demonstrate alternating gradient descent is provably not locally asymptotically stable in optimizing the GAN formulation of PCA. We diagnose the problem as the minimax duality gap being non-zero, and propose a new GAN architecture whose duality gap is zero, where the value of the game is equal to the previous minimax value (not the maximin value). We prove the new GAN architecture is globally asymptotically stable in optimization under alternating gradient descent.

==> conclusion.tex <==
\section{Conclusion and Future Work}

In this paper, we proposed a principled way for designing GAN that achieves optimal generalization property and is stable in degenerate case. Our theory demonstrates a exponential to polynomial sample complexity gap from naive GAN structure to projection under weakened distance structure. We also propose a way to test the strength of discriminator, which makes our theory more applicable in practice. 

It is worth pointing out that there is still much work left. We are working to generalize the analysis to neural network generators to derive a scheme that is both statistically optimal and computationally efficient.  Viewing GANs as a promising novel technique of unsupervised learning, it is also of interest to study the performance of GANs when they are applied to specific data distributions, and to analyze whether one can show provable guarantees for the induced optimization problem. Given the outstanding empirical performance of reconstructing images and texts, we shall expect that GANs are capable of near-optimally learn and reconstruct simple structures like mixture of subspaces or Gaussian distributions. We also propose to explore the relationships between the alternative gradient algorithm of GANs and existing algorithms of unsupervised learning, such as the lossy data compression inspired algorithm~\cite{yang2008unsupervised}.  

On the other hand, the formulation issue of GAN remains unsolved in our paper. It is still unclear if Wasserstein or other metrics are the best discrepancy measure for different tasks. And the evaluation of GAN is significantly related to the formulation task. Also, we believe GAN is able to deal with multiple perturbations in different distance as a robust estimator.


==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}
The goal of GANs is to output a generator $g(\cdot)$ from some generator family $\cG$. The generator function takes Gaussian random noise $Z \sim \mathcal{N}(\mathbf{0},\mathbf{I}_r)$ as input and outputs another random variable which is as close as possible to the real distributions of images or texts. In order to characterize the 'closeness' between distributions, we need to choose a \emph{population} distance function $L(\cdot,\cdot)$ from domain specific knowledge. The ultimate goal is to find the generator that is closest to the real distribution $\bbP_X$ under the distance function $L(\cdot,\cdot)$, i.e.

\begin{equation}
%\label{equ:formulation}
   {\hat g} = \argmin_{g\in\cG}L(g({Z}), \bbP_X)
\end{equation}



The formulation in equation (\ref{equ:formulation}) suggests that we project the real distribution $\bbP_X$ onto the generator family $\cG$ under distance $L$. However, it is unclear how to choose distance function $L$ and the generator family $\cG$. As a concrete example, the vanilla GAN~\cite{goodfellow2014generative} defines the distance function $L$ as the Jensen-Shannon divergence, and uses neural network as generator family. A general principle is to choose $L$ and $\cG$ such that there exists a generator in the generator family, which is close enough to the real distribution under distance $L$. %More concretely, by choosing $L$ and $\cG$, we hope to make the oracle error term $\inf_{g(\cdot)\in \mathcal{G}} L(\bbP_{g(Z)},\bbP_X) $ in equation (\ref{eqn:generalization}) as small as possible, otherwise it is hard to learn an appropriate approximation.

It is also natural to interpret the requirements in the form of robustness in generative modeling with respect to problem specific perturbation models. We provide two ways of interpretation in the discussion section.
\begin{itemize}
    \item When the real distribution is in the generator family, we are assuming $L$ is an appropriate distance function to compare between generator families.
    \item 
\end{itemize}

\begin{itemize}
    \item When the real distribution is in the generator family, we are assuming $L$ is an appropriate distance function to compare between generator families. For example, total variation distance is meaningless if the support of two generators does not match. Similar problem exists for Kullback-Leibler divergence. This was also observed in~\cite{arjovsky2017wasserstein} where the authors compared the Jensen-Shannon divergence and the coupling induced distances such as the Wasserstein distance, and showed that the Wasserstein distance provides meaningful measures for discrepancies between distributions even when the dimension of generated distribution is smaller than that of the true distribution. An illustrating example is learning a $2$-D distribution with $1$-D generator family. As is shown in the left figure in Fig.\ref{fig:twogenerator}, the two generators are equally bad under Jensen-Shannon divergence, while apparently generator one is a better approximation. When learning a high dimensional distribution with low dimensional generator, one should try to find a good perturbation model to capture it, which is in fact determined by the distance function $L$. %Unless the two Gaussians are totally the same, their total variation distance is always $1$, while Wasserstein distance is able to characterize the distance meaningfully. 
    \item When the real distribution is not in the generator family, we can interpret GAN from a robust statistic's point of view. The choice of $L$ is determined by the assumption that the real distribution is one of the generator perturbed under certain distance.
    It was shown in~\cite{gao2018robust} that various formulation of GAN, including TV-GAN and JS-GAN~\cite{nowozin2016f,goodfellow2014generative}, can all lead to statistically optimal robust estimators for the parameters of interest under Huber's contamination model~\cite{huber1964robust}, which assumes $\epsilon$ fraction of data is corrupted by adversary. In fact, as long as the distance function $L$ satisfies triangle inequality, one can easily show robustness guarantee using a similar argument this paper describes. However, Huber's contamination model is based on perturbation under total variation distance between distributions, which also suffers from support mismatch.  Meanwhile, under Huber's model, Wasserstein distance can be huge since Wasserstein distance takes into consideration the geometry distance. For the sake of robustness, one should be clear about under what perturbation the data could be corrupted. It is still poorly understood how to formulate multiple perturbation model and how to design corresponding GAN structures.
\end{itemize}



Based on above discussion, we find that in nature, the perturbation may come from different sources, while no single distance function can characterize all of the perturbations well. As is shown in the right figure in Fig.\ref{fig:twogenerator}, if the observed distribution is a 2-D distribution perturbed an $\epsilon$ fraction under TV distance, and the generator is all 1-D distribution, both Wasserstein distance and total variation distance will be huge. It is meaningless to minimize any of the two single distance under this case. Thus we propose a cascaded GAN structure, which is able to characterize different perturbation model. 


\begin{align}
    \min_{g \in \cG,g' \in \cG'} d_{TV}(\bbP_X , \bbP_{g(Z)}) + \lambda W_p(\bbP_{g(Z)},\bbP_{g'(Z)})
\end{align}

In a more general case, $d_{TV}$ and $W_p$ can be replaced by any distance function. The $TV$-$W_2$ combination is similar to the setting of robust PCA~\cite{candes2011robust} and compressive outlier sensing~\cite{li2015identifying}, where the data matrix is decomposed into a low rank matrix plus sparse noise perturbation. The target is to minimize the rank of low rank matrix along with the sparsity of the noisy matrix, with the constraint that they sum up to the original matrix. Compressive outlier sensing can be a special case of the cacaded GAN structure, where the low rank property is constrained in the choice of $\cG'$ and $W_2$ distance, and the sparsity is controlled by the total variation distance.
The chained tv and W2 perturbation problem can also be solved by optimizing GAN with a new distance function $d = \inf_\pi \bbE [\min(||X-Y||^2, {\bf 1}_{X\neq Y})]$. However, this would require a new design of GAN, while the cascaded GAN structure can be optimal by simply combining two different GANs.  AmbientGAN~\cite{bora2018ambientgan} is also able to solve chained perturbation model, but requires the knowledge of the exact formulation of the second perturbation.

The choice of distance function should also reflect the desirable properties of downstream applications of the output generator of trained GANs. For example, the \emph{Inception Score}~\cite{barratt2018note}, which is intrinsically \emph{mutual information} between input and output for a fixed channel, is raised as one potential measure for quality of a generative model, but it fails to distinguish between the good generator that has well approximated the true image distribution and the naive generator that simply samples the training data uniformly at random. \emph{Fr\'echet Inception Distance} (FID)~\cite{heusel2017gans} uses the similar idea to compute the Wasserstein-2 distance between moment-matching Gaussians from the coding layer of Inception network, which is shown to be more robust to noise and achieve better performance than inception score for images. From robustness point of view, FID is assuming that the features of real distribution is close to that of generator family in the coding layer, which might be more reasonable than other distance functions. Another assessment measure is precision and recall~\cite{sajjadi2018assessing}, which disentangles the divergence into two separate components, the overlap between distributions and its complement. It is able to effectively quantify the degree of mode dropping and mode inventing on real world data sets. Another line of work uses a statistical hypothesis testing framework called maximum mean discrepancy as loss function. Training to minimize this discrepancy can be interpreted as matching all moments of the model distribution to the empirical data distribution~\cite{li2015generative}.

The choice of $L$ and $\cG$ heavily depends on our domain specific knowledge of the true distribution. For given generator family and distance function $L$, it is also of great importance to study the statistical and optimization properties. In the Gaussian example~\cite{feizi2017understanding}, the Wasserstein-2 distance $W_2$ and linear generator family are adopted for learning a Gaussian distribution since it exactly recovers PCA as the best $k$-dimensional Gaussian covariance matrix approximation of a full $d$-dimensional Gaussian distribution. In our paper, we propose to further study the case of $W_2$ and Gaussian, and extend this to $W_\mathcal{F}$ distance and general real distributions. We do not think in practice one should use $W_2$ or use Gaussian generator, but it is a good example that exactly implements the formulation idea proposed and provides insight for general GAN design. For more general real distribution, we discuss $W_\mathcal{F}$ distance, which also has a very nice interpretation of looking at the gaps between the expectations of some test functions $f$ under two distributions.  
%hence in this paper we assume that $L$ is given a priori, and our goal is to identify the generator whose output distribution is the \emph{closest} to the real distribution under the pre-specified distance $L$. 


\subsection{Relationship to Mode Collapse}
In fact, any of the three aspects, formulation, generalization and optimization can be the potential causes of the problems of mode collapse. In the formulation setting, if the generator is set to be too weak, or the discriminator is set to be too strong, then the oracle term is huge, thus the learned distribution is far from true distribution. Generator is not able to learn a meaningful distribution. In the statistical setting, perhaps not weakened well enough so still find another suboptimal distribution. In the optimization setting, it may just not be able to optimize. But we say if people follow our principled way of thinking, there is good chance to diagnose GANs. In particular, we already provided ideas to test distance strengths.

==> formulation.tex <==
\section{Formulation of GANs}
Based on the interpretation of equation (\ref{eqn:generalization}) and the understanding of perturbation under different sources, we propose a method that cascades different types of GANs together so that the distance is able to detect different perturbations and recover precisely the optimal generator. This procedure can be summarized in the following Theorem.

\begin{theorem}
\label{thm:cascaded}
Assume we are doing projection under weakened distance for total variation distance and $W_2$ distance, i.e., there exists two algorithms
\begin{align}
    \hat g_1 = \argmin_{g\in\cG_1} \tW_2(\bbP_{g(Z)},\hat \bbP_X^n) \\
    \hat g_2 = \argmin_{g\in\cG_2} \tilde{d}_{TV}(\bbP_{g(Z)},\hat \bbP_X^n)
\end{align}
such that
\begin{align}
    W_2(\bbP_{\hat g_1(Z)},\bbP_X) \leq \inf_{g\in \cG_1} W_2(\bbP_{g(Z)},\bbP_X) + \epsilon_1 \\
    d_{TV}(\bbP_{\hat g_2(Z)},\bbP_X) \leq \inf_{g\in \cG_2} d_{TV}(\bbP_{g(Z)},\bbP_X) + \epsilon_2 
\end{align}
Then for
\begin{align}
    \hat g_1, \hat g_2 = \argmin_{g_1 \in \cG_1,g_2 \in \cG_2}  W_2(\bbP_{g_1(Z)},\bbP_{g_2(Z)}) + \tilde{d}_{TV}(\bbP_X , \bbP_{g_2(Z)}) 
\end{align}
We have 
\begin{align}
    W_2(\bbP_{\hat g_1},\bbP_{\hat g_2(Z)})+ {d}_{TV}(\bbP_X , \bbP_{\hat g_2(Z)}) \leq \epsilon_1 + \epsilon_2 + 
\end{align}
\end{theorem}

%Assume two different are operating under distance function $L_1$, $L_2$






\begin{comment}
\subsection{Preliminary results}

In the Gaussian example~\cite{feizi2017understanding}, the PIs aim at proposing a divergence function to measure the distance between two Gaussian distributions. The Wasserstein-2 distance $W_2$ is adopted, due to the following reasons: 
\begin{itemize}
    \item it was shown in~\cite{feizi2017understanding} that the best $k$-dimensional Gaussian approximation of a full $d$-dimensional Gaussian distribution under $W_2$ is the Gaussian distribution whose covariance is the $k$-PCA of the original Gaussian. Hence, from a population point of view, $W_2$ recovers the PCA, arguably one of the most popular unsupervised learning algorithms;
    \item the primal form of $W_2$ can be viewed as a coupling approach under squared error loss function. From an optimal transport point of view, $W_2$ is measuring the minimum cost of transporting one Gaussian distribution to the other, while the cost function is the quadratic function of the transportation distances. Since Gaussian distributions are completely characterized by the mean and covariance, it was shown that the squared error loss function is particularly compatible with Gaussian distributions~\cite{givens1984class}. 
\end{itemize}

\subsection{Proposed research}


\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{figformulation.png}
\caption{An illustration of the proposed formulation (discrepancy measure) of GANs induced by different population goals.  }
\label{fig:formulation}
\end{figure}

As is shown in Figure \ref{fig:formulation}, we focus on the fomulation of GAN indcued by three aspects: robustness requirement, application scenarios and feature extraction.

\subsubsection{Task 1: Robustness under general corruption models}

In practice, one can never ensure that the true distribution can be exactly represented by one of the generators. Hence, it is crucial to obtain a \emph{robust} GAN, which asserts that if the true distribution is not too \emph{far} from the family of generators, the GANs output should be a reasonable approximation of the true distribution. 

The key to the reasoning above lies in the definition of being ``\textbf{not too far}". It is intimately related to the field of robust statistics, where one assumes that the observations are corrupted versions of samples from the true distribution. If one considers the corruption model as the Huber contamination model~\cite{huber1964robust}, where $\epsilon$ fraction of input sample data is corrupted and substituted with samples from an arbitrarily chosen adversarial distribution, then being ``not too \textbf{far}'' has a precise meaning: \textbf{being close under the total variation distance}. 

However, it is not always true that the Huber contamination model captures the essence of data corruption in practical applications. For example, consider two one-dimensional Gaussian distribution in two dimensions. If the supports of these two distributions do not match, then the total variation distance between them is always one---the maximal possible value. From this perspective, in applications where one views the slight rotation of the support of a Gaussian as generating a \textbf{close-by} distribution to the original Gaussian, measuring the closeness under the total variation distance is \emph{not} appropriate. This was also observed in~\cite{arjovsky2017wasserstein} where the authors compared the Jensen--Shannon divergence and the coupling induced distances such as the Wasserstein distance, and showed that the Wasserstein distance provides meaningful measures for discrepancies between distributions even when the dimension of generated distribution is smaller than that of the true distribution.

We propose to formulate GANs based on general corruption models that are more general than the Huber contamination model. In the specific cases of estimating Gaussian mean, covariance, and regression, it was shown in~\cite{gao2018robust} that there exist various formulations of GANs~\cite{nowozin2016f,goodfellow2014generative} that all lead to provably robust estimators for the parameters of interest. We propose to study data corruption models that are more general than studied in the literature, and precisely characterize the family of GANs formulations whose solutions satisfy robustness properties under specific corruption models. 

\subsubsection{Task 2: Application driven formulation}

We believe the formulation of GANs should reflect the desirable properties of downstream applications of the output generator of trained GANs. GANs have been successfully applied for a large variety of applications, e.g., conditional GAN~\cite{mirza2014conditional, isola2017image} and cycle GAN~\cite{zhu2017unpaired} for style transfer, Defense-GAN~\cite{samangouei2018defense} for defensing against adversarial examples and other GAN structures for compressed sensing~\cite{bora2017compressed}. The formulation and evaluation of GANs should be able to distinguish between generators that perform well or badly in these applications. For example, if the generator is only able to memorize the training samples, and would only uniformly sample one of the training samples when it is queried, the appropriate formulation of GANs should point out that it is a \textbf{bad} generator since it cannot perform the task of style transfer as in~\cite{isola2017image}. 

Naturally as it seems, the widely used evaluation metrics of GANs sometimes fail to capture the properties mentioned above. For example, the \emph{Inception Score}~\cite{barratt2018note}, which is intrinsically \emph{mutual information} between input and output for a fixed channel, is raised as one potential measure for quality of a generative model, but it fails to distinguish between the good generator that has well approximated the true image distribution and the naive generator that simply samples the training data uniformly at random. 

We propose to conduct a systematic study of GANs formulations to distill the key requirement of GANs for successful downstream applications. We plan to significantly generalize existing literature~\cite{poole2016improved, lucic2017gans, kurach2018gan, shmelkov2018good,borji2018pros} and propose novel formulations driven by the ever-growing applications of GANs. 


\subsubsection{Task 3: Incorporating knowledge via feature extraction}

Motivated by the Gaussian example~\cite{feizi2017understanding}, we consider the formulation of GANs using coupling induced distances. The naturalness of the Wasserstein-2 distance for Gaussian distributions is closely related to the naturalness of measuring the cost of transporting Gaussian mass from one distribution to the other using quadratic functions. However, it may no longer be appropriate to use squared error loss functions to quantify the distances between difference images. We propose to incorporate the knowledge about specific data sets through feature extraction. Indeed, the key reason for the success of the style transfer~\cite{gatys2015neural} is that the features extracted by middle layers of the VGG network provides a meaningful representation of the \emph{style} of the image. Hence, we propose to explore natural distances on the feature spaces of natural images/texts, and use those to formulate GANs in order to incorporate the local geometry and metric properties of real data. Our goal is to find ways to incorporate prior knowledge about the data set in GANs design to capture the qualitative visual quality of generative models. 
\end{comment}
